Fairness in Reinforcement Learning

We initiate the study of fairness in reinforcement learning, where the actions of a learning algorithm may affect its environment and future rewards. Our fairness constraint requires that an algorithm never prefers one action over another if the long-term (discounted) reward of choosing the latter action is higher. Our first result is negative: despite the fact that fairness is consistent with the optimal policy, any learning algorithm satisfying fairness must take time exponential in the number of states to achieve non-trivial approximation to the optimal policy. We then provide a provably fair polynomial time algorithm under an approximate notion of fairness, thus establishing an exponential gap between exact and approximate fairness

==> figure <==

\begin{figure}%[h]
\centering
\begin{minipage}[c]{.5\textwidth}
\includegraphics[width=0.9\textwidth]{not-myopic.png}
%\scalebox{.55}{
%\begin{tikzpicture}
%[every node/.style={circle, fill=white, draw=black, minimum size=1.3cm}]
%\node (1) at  (-6, 0){$s_1, 0.5$};\node (2) at (-3,0){$s_2, 0$};\node (3) at (0, 0){$s_3, 0$};\node (4) at (3, 0){$s_4, 1$};
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (1) [out=330,in=210]  to (2);\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (2)  to (3);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]  (1) [out=245,in=295] to (1);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (3) [out=245,in=295] to (3);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (2) [out=150,in=30] to (1);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (3) to (4);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (4) [out=245,in=295] to (4);
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (-4.5,-1.7) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (-1.5,-0.25) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (1.5,-0.25) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (0,-1.9) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (-6,-1.9) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (-4.5,0.1) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L, R}] at (3.05,-1.9) {};
%\end{tikzpicture}}
\end{minipage}
\quad
\quad
\quad
\begin{minipage}[c]{.5\textwidth}
\centering
\caption{An MDP where optimal policy is not myopic.  States are
  represented by circles (text inside denote the state name and the
  deterministic reward). The arrows from the states denote the two
  possible actions $L$ and $R$ in each state.  In $s_1$ and $s_2$
  actions with lower rewards will finally result in higher rewards in
  the future (which is achievable after arriving in $s_4$).
  \label{fig:greedy}}
\end{minipage}
\end{figure}


==> missing-proofs-fairness.tex <==
\iffalse
\subsection{Omitted Proofs for Section~\ref{sec:fairness}}
\label{sec:missing-proofs-fairness}

\begin{proof}[Proof of Observation~\ref{obs:exact-opt}]
  In time $t$, let state $s_t$ denote the state from which $\pi$
  chooses an action.  Let $a^* = \argmax_a Q_M^*(s_t, a)$ and
  $A^*(s_t) = \{a \in A \mid Q_M^*(s_t, a) = Q_M^*(s_t, a^*)\}$.  The
  policy of playing an action uniformly at random from $A^*(s_t)$ in
  state $s_t$ for all $t$, is fair and optimal.
\end{proof}

\begin{proof}[Proof of Observation~\ref{obs:approx-fair}]
  Assume that $\pi^*$ is not \afair fair.  Given state $s$, the
  action that $\pi^*$ takes from $s$ is uniquely determined since
  $\pi^*$ is deterministic, so we may denote it by $a^*$.  Then there
  exists a time step in which $\pi^*$ is in state $s$ and chooses
  action $a^*(s)$ such that there exists another action $a$ with
\[
	Q^*_M(s, a) > Q^*_M(s, a^*(s)) + \alpha,
\] 
a contradiction of the optimality of $\pi^*$. 
\end{proof}

\begin{proof}[Proof of Observation~\ref{obs:random-walk}]
  Let $\alg$ denote an algorithm that in every state plays uniformly
  at random between all available actions. Then
  $\alg(s, \hist_{t-1})_a = \alg(s, \hist_{t-1})_{a'}$ regardless of
  state $s$, (available) action $a$, or history $h_{t-1}$.
  $Q^*_M(s,a) > Q^*_M(s,a') + \alpha \Rightarrow \mathcal{L}(s,
  \hist_{t-1})_a \geq \mathcal{L}(s, \hist_{t-1})_{a'}$
  then follows immediately, which guarantees both fairness and
  \afair fairness.
\end{proof}

\begin{proof}[Proof of Observation~\ref{obs:m-alphaa}]
  Assume $\pi$ is not $\alpha$-action fair. Then there must exist round $t$,
  state $s$, and action $a$ such that
  $Q^*_M(s,a) > Q^*_M(s,a') + \alpha$ and
  $\mathcal{L}(s, \hist_{t-1})_a < \mathcal{L}(s,
  \hist_{t-1})_{a'}$.
  Therefore $\mathcal{L}(s, \hist_{t-1})_{a'} > 0$, so $M^{\alpha}$
  must include action $a'$ from state $s$. But this is a
  contradiction, as in state $s$ $M^{\alpha}$ only includes actions
  $a'$ such that $Q^*_M(s,a') + \alpha \geq Q^*_M(s,a)$. $\pi$ is
  therefore $\alpha$-action fair.
\end{proof}

\begin{proof}[Proof of Observation~\ref{obs:m-alpha-opt}]
  If $\pi^*$ is not optimal in $M$, then there exists a state $s$ and
  action $a$ such that
  $Q^*_M(s, a) > \E_{a^*(s)\sim\pi^*(s)} Q^*_M(s, a^*(s))$ where
  $a^*(s)$ is drawn from $\pi^*(s)$ and the expectation is taken over
  choices of $a^*(s)$. This is a contradiction because action $a$ is
  available from state $s$ in $M^\alpha$ by
  Definition~\ref{def:fair-mdp}.
\end{proof} 

\fi

==> non-myopic-fig.tex <==

\begin{figure}%[h]
\centering
\begin{minipage}[c]{.5\textwidth}
\includegraphics[width=0.9\textwidth]{not-myopic.png}
%\scalebox{.55}{
%\begin{tikzpicture}
%[every node/.style={circle, fill=white, draw=black, minimum size=1.3cm}]
%\node (1) at  (-6, 0){$s_1, 0.5$};\node (2) at (-3,0){$s_2, 0$};\node (3) at (0, 0){$s_3, 0$};\node (4) at (3, 0){$s_4, 1$};
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (1) [out=330,in=210]  to (2);\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (2)  to (3);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}]  (1) [out=245,in=295] to (1);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (3) [out=245,in=295] to (3);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (2) [out=150,in=30] to (1);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (3) to (4);
%\draw[decoration={markings,mark=at position 1 with
%    {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (4) [out=245,in=295] to (4);
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (-4.5,-1.7) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (-1.5,-0.25) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={R}] at (1.5,-0.25) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (0,-1.9) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (-6,-1.9) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L}] at (-4.5,0.1) {};
%\node [draw,rectangle,color=white,minimum width=0.01cm,minimum height=0.01cm,label={L, R}] at (3.05,-1.9) {};
%\end{tikzpicture}}
\end{minipage}
\quad
\quad
\quad
\begin{minipage}[c]{.5\textwidth}
\centering
\caption{An MDP where optimal policy is not myopic.  States are
  represented by circles (text inside denote the state name and the
  deterministic reward). The arrows from the states denote the two
  possible actions $L$ and $R$ in each state.  In $s_1$ and $s_2$
  actions with lower rewards will finally result in higher rewards in
  the future (which is achievable after arriving in $s_4$).
  \label{fig:greedy}}
\end{minipage}
\end{figure}


==> techniques.tex <==

\subsection{Our Techniques}\label{sec:techniques}


We now briefly describe the tools we use to prove the theorems
described above. The lower bounds follow from constructing two similar
MDPs and arguing that fair and \pfair fair algorithms must behave
identically for both until receiving some observation distinguishing
the two, which will take an exponential number of steps in the size of
state space with constant probability.

We then study a different relaxation of fairness, called \afair
fairness, which allows an algorithm to prefer slightly worse actions
to slightly better ones.  We adapt \ecube~\citep{KearnsS02}, a
well-known algorithm for MDP learning, to satisfy \afair
fairness. \ecube transitions between exploration and exploitation: if
some state has not been sufficiently explored, \ecube takes the least
explored action in that state.  The pigeonhole principle then implies
\ecube will eventually explore some state often enough to learn
accurate estimates of its reward and transition functions, after which
\ecube treats the state as ``known''.  To exploit, \ecube treats the
set of known states as if they are the only states of the MDP and
follows a near-optimal policy if such a policy exists in the MDP
restricted to the known states. Otherwise, \ecube plans to
\emph{escape} to the set of ``unknown" states in hopes of achieving
better long-term rewards.

Developing a fair version of \ecube requires a number of nontrivial
modifications to both the algorithm and its analysis. The first main
one has to do with the definition of a known state. The original
\ecube uses a weak definition that is sufficient for one-step
lookahead. Since fairness demands that an algorithm {\em never\/}
prefer a much worse action, we require a much stronger definition of
known state for \ecubep that permits accurate estimation of
$Q^*$ values (long-term discounted rewards) rather than just
next-state transitions.

The second major modification arises from the fact that when
attempting to escape to unknown states, \ecube may badly violate
fairness, since it is ignoring rewards entirely in an attempt to reach
rarely visited states.  \ecubep tries to find an escape policy subject
to our fairness constraint. A ``win-win'' analysis proves that
whenever \ecubep cannot execute an ``exploit'' policy, then there must
exist a \emph{fair} escape policy, and so our algorithm is always
either able to exploit or fairly escape when it encounters a known
state.

\iffalse First, in the unknown states, \ecube favors actions which
have yet to be explored, which may or may not have higher long-term
rewards than their alternatives.  Second, while following a policy to
escape to the unknown states, \ecube might potentially favor actions
with lower long-term rewards.  For the first problem, \ecubep employs
random exploration.  To remedy the second problem, \ecubep computes
and follows an escape policy in a restricted MDP in which only actions
with long-term reward close to the optimal choice are available. This
behavior guarantees \afair fairness.  However, to compute such a
restricted MDP \ecubep requires a stronger notion of known states
compared to \ecube and this in turn increases the running time of
\ecubep compared to \ecube.  \fi
%
%, as .  Hence, \ecubep
%restricts all MDPs it considers to only having those
% on the \emph{exploration} MDP which treats
%unknown states as having reward $1$ and known states as having reward
%$0$. If this policy reaches an unknown state with high enough
%probability, this serves as a proof to the algorithm that an optimal
%policy must reach an unknown state quickly --- it is therefore fair to
%follow the optimal policy for the exploration MDP.
%
%

